DiagNet: towards a generic, Internet-scale root cause analysis solution

Diagnosing problems in Internet-scale services remains particularly difficult and costly for both content providers and ISPs. Because the Internet is decentralized, the cause of such problems might lie anywhere between an end-user's device and the service datacenters. Further, the set of possible problems and causes is not known in advance, making it impossible in practice to train a classifier with all combinations of problems, causes and locations. In this paper, we explore how different machine learning techniques can be used for Internet-scale root cause analysis using measurements taken from end-user devices. We show how to build generic models that (i) are agnostic to the underlying network topology, (ii) do not require to define the full set of possible causes during training, and (iii) can be quickly adapted to diagnose new services. Our solution, DiagNet, adapts concepts from image processing research to handle network and system metrics. We evaluate DiagNet with a multi-cloud deployment of online services with injected faults and emulated clients with automated browsers. We demonstrate promising root cause analysis capabilities, with a recall of 73.9% including causes only being introduced at inference time.

==> data_family_recall_csv.tex <==
i,family,forest,forest_err,gaussian,gaussian_err,diagnet,diagnet_err,hybrid3,hybrid3_err,hybrid3p,hybrid3p_err
1,download,0.821,0.022,0.000,0.000,0.773,0.027,0.762,0.041,0.901,0.015
2,rtt,0.594,0.000,0.028,0.000,0.495,0.019,0.568,0.032,0.753,0.017
3,loss,0.759,0.000,0.032,0.000,0.313,0.020,0.476,0.038,0.740,0.015
4,jitter,0.764,0.001,0.061,0.000,0.229,0.033,0.358,0.035,0.726,0.013
5,net-edge,1.000,0.000,0.000,0.000,0.865,0.064,0.851,0.061,0.998,0.003
6,load,1.000,0.000,0.000,0.000,0.977,0.006,0.982,0.004,0.995,0.002


==> data_history_0_csv.tex <==
epoch,train_loss,val_loss
0,0.354624,0.274126
1,0.236584,0.208284
2,0.197016,0.186607
3,0.185817,0.176227
4,0.170220,0.169681
5,0.163162,0.159776
6,0.152783,0.147176
7,0.155680,0.143843
8,0.145024,0.144422
9,0.137300,0.144179
10,0.130739,0.134853
11,0.123710,0.133284
12,0.120811,0.130051
13,0.119998,0.132777
14,0.114136,0.131098
15,0.109892,0.128007
16,0.107254,0.120463
17,0.111880,0.122968
18,0.105459,0.116824
19,0.100727,0.121286
20,0.101196,0.115931
21,0.094224,0.116822
22,0.095419,0.119597
23,0.092588,0.112410
24,0.088319,0.112530
25,0.091051,0.113214
26,0.085447,0.110755
27,0.082918,0.114705
28,0.077513,0.110875
29,0.076912,0.108662
30,0.079904,0.107521
31,0.074464,0.107155
32,0.074556,0.107949
33,0.074341,0.108283
34,0.072036,0.103438
35,0.069383,0.106782
36,0.068927,0.106907
37,0.069373,0.112321
38,0.066800,0.105073
39,0.066153,0.104768
40,0.064039,0.110391
41,0.061478,0.108405
42,0.058083,0.111276
43,0.058407,0.108240
44,0.057058,0.108254
45,0.058382,0.104446
46,0.060300,0.109009
47,0.056622,0.108798
48,0.056309,0.107730
49,0.056000,0.110513


==> data_history_10_csv.tex <==
epoch,train_loss,val_loss
0,0.146398,0.121466
1,0.091496,0.094940
2,0.080349,0.086069
3,0.070354,0.074247
4,0.066832,0.079245
5,0.054823,0.053266
6,0.050232,0.072539
7,0.047175,0.063231
8,0.042223,0.058865
9,0.040797,0.064679
10,0.036688,0.063062
11,0.035761,0.054954
12,0.031858,0.056750
13,0.033296,0.055790
14,0.031035,0.059909
15,0.038133,0.069123
16,0.037312,0.052771
17,0.029115,0.054203
18,0.027414,0.056355
19,0.027187,0.054084
20,0.026889,0.060393
21,0.024712,0.052807
22,0.024022,0.057733
23,0.022870,0.054041
24,0.022024,0.063153
25,0.022090,0.059845
26,0.021072,0.061553
27,0.019872,0.062282
28,0.018609,0.061643
29,0.019059,0.060148
30,0.017799,0.068745
31,0.017659,0.060915
32,0.017062,0.058208
33,0.017022,0.061829
34,0.015856,0.061876
35,0.016260,0.063863
36,0.019983,0.070606
37,0.018304,0.061659
38,0.016728,0.063040
39,0.015940,0.062458
40,0.015138,0.062514
41,0.014700,0.063656
42,0.014201,0.066558
43,0.014026,0.066736
44,0.014116,0.064668
45,0.013642,0.066403
46,0.013534,0.066757
47,0.014559,0.068452
48,0.013720,0.070976
49,0.012856,0.067057


==> data_history_13_csv.tex <==
epoch,train_loss,val_loss
0,0.056441,0.026130
1,0.026680,0.017532
2,0.027507,0.016784
3,0.036884,0.020288
4,0.024461,0.016422
5,0.020354,0.012772
6,0.017540,0.014820
7,0.016423,0.016000
8,0.015290,0.012418
9,0.015263,0.010826
10,0.013590,0.010610
11,0.013516,0.013050
12,0.013897,0.013083
13,0.011755,0.014003
14,0.011688,0.018690
15,0.012371,0.013838
16,0.011730,0.013738
17,0.010820,0.014323
18,0.011814,0.013778
19,0.011073,0.015264
20,0.010505,0.015438
21,0.008957,0.014724
22,0.009031,0.014595
23,0.008572,0.014210
24,0.008973,0.012043
25,0.008555,0.013649
26,0.008468,0.014176
27,0.009169,0.015203
28,0.008238,0.013192
29,0.008732,0.015016
30,0.008630,0.012247
31,0.008240,0.014493
32,0.008078,0.013710
33,0.007188,0.014159
34,0.007046,0.012533
35,0.007031,0.016370
36,0.007336,0.012909
37,0.006864,0.013759
38,0.006551,0.013605
39,0.007498,0.013743
40,0.006295,0.013583
41,0.006359,0.014869
42,0.005985,0.014965
43,0.006195,0.012375
44,0.006575,0.014051
45,0.005973,0.013477
46,0.005846,0.014725
47,0.005451,0.015721
48,0.006245,0.014611
49,0.005574,0.014213


==> data_history_14_csv.tex <==
epoch,train_loss,val_loss
0,0.130263,0.081206
1,0.095016,0.073025
2,0.078807,0.062854
3,0.067848,0.063146
4,0.063693,0.066695
5,0.065471,0.062133
6,0.056708,0.061491
7,0.055628,0.064240
8,0.053014,0.061259
9,0.050741,0.063827
10,0.052388,0.058821
11,0.051839,0.062191
12,0.050845,0.058682
13,0.047709,0.058709
14,0.044716,0.045962
15,0.039796,0.045163
16,0.040343,0.056801
17,0.038733,0.050613
18,0.037644,0.047545
19,0.036400,0.050424
20,0.035923,0.051369
21,0.034171,0.053235
22,0.034176,0.052905
23,0.033611,0.055551
24,0.033177,0.058177
25,0.032381,0.055820
26,0.031405,0.053283
27,0.030558,0.058210
28,0.029453,0.054211
29,0.028442,0.050638
30,0.028288,0.051098
31,0.027744,0.054344
32,0.026886,0.052005
33,0.027387,0.056323
34,0.026951,0.053665
35,0.027484,0.051510
36,0.025993,0.052948
37,0.025234,0.054768
38,0.024482,0.054791
39,0.024750,0.055322
40,0.024157,0.055850
41,0.023088,0.055171
42,0.022962,0.067047
43,0.023991,0.063699
44,0.023635,0.054954
45,0.022169,0.055693
46,0.022233,0.062075
47,0.023500,0.063199
48,0.023176,0.058513
49,0.021008,0.062076


==> data_history_5_csv.tex <==
epoch,train_loss,val_loss
0,0.096675,0.057879
1,0.054870,0.049541
2,0.048295,0.042522
3,0.042670,0.042630
4,0.041255,0.038080
5,0.038139,0.045576
6,0.035351,0.036986
7,0.032424,0.045982
8,0.031581,0.047457
9,0.030055,0.039418
10,0.026820,0.044854
11,0.025296,0.046840
12,0.023256,0.043726
13,0.021656,0.047082
14,0.020860,0.054420
15,0.020551,0.040301
16,0.021809,0.042206
17,0.020571,0.042304
18,0.018428,0.045420
19,0.019158,0.043060
20,0.017595,0.046210
21,0.016664,0.042163
22,0.015130,0.040470
23,0.014961,0.053320
24,0.015207,0.046495
25,0.015632,0.048635
26,0.014154,0.056792
27,0.017527,0.045441
28,0.014825,0.047811
29,0.013495,0.042572
30,0.012728,0.045529
31,0.011866,0.046934
32,0.011648,0.046768
33,0.011884,0.051270
34,0.012053,0.049771
35,0.011529,0.049722
36,0.011057,0.054462
37,0.009512,0.049003
38,0.009559,0.055498
39,0.009323,0.054530
40,0.009782,0.055045
41,0.008815,0.054792
42,0.008196,0.053111
43,0.008748,0.060741
44,0.008704,0.055013
45,0.007926,0.052986
46,0.008148,0.056941
47,0.009247,0.065007
48,0.007281,0.056427
49,0.007388,0.057990


==> data_history_6_csv.tex <==
epoch,train_loss,val_loss
0,0.154115,0.123855
1,0.114814,0.111740
2,0.101767,0.087376
3,0.079603,0.087559
4,0.074887,0.082065
5,0.068232,0.071793
6,0.066047,0.076097
7,0.064484,0.073724
8,0.058704,0.067917
9,0.058186,0.068947
10,0.053590,0.068819
11,0.050918,0.066224
12,0.050482,0.066491
13,0.049001,0.069329
14,0.047225,0.070534
15,0.044731,0.070667
16,0.043679,0.067019
17,0.041930,0.065772
18,0.040668,0.069730
19,0.038635,0.066526
20,0.037909,0.070626
21,0.037256,0.068368
22,0.037281,0.070455
23,0.036751,0.070944
24,0.035571,0.065100
25,0.034237,0.071309
26,0.033248,0.068917
27,0.032399,0.067051
28,0.031453,0.066662
29,0.031242,0.073038
30,0.030945,0.070521
31,0.029370,0.066916
32,0.029295,0.073294
33,0.028652,0.069124
34,0.028926,0.071027
35,0.028569,0.068753
36,0.027376,0.073072
37,0.027579,0.072884
38,0.027410,0.071761
39,0.026229,0.075942
40,0.025836,0.074606
41,0.025144,0.070720
42,0.024649,0.069690
43,0.024154,0.079132
44,0.024396,0.068716
45,0.025449,0.075681
46,0.024248,0.075851
47,0.023272,0.073714
48,0.023067,0.073378
49,0.022432,0.072362


==> data_history_7_csv.tex <==
epoch,train_loss,val_loss
0,0.066634,0.042671
1,0.031432,0.030380
2,0.023295,0.027077
3,0.015373,0.027718
4,0.012546,0.020405
5,0.013965,0.023793
6,0.011249,0.022810
7,0.008720,0.020577
8,0.009772,0.020419
9,0.007426,0.022897
10,0.007117,0.024870
11,0.006146,0.023691
12,0.006027,0.025142
13,0.006399,0.024467
14,0.007611,0.026511
15,0.006632,0.024562
16,0.005380,0.026550
17,0.005024,0.023927
18,0.004758,0.024598
19,0.004745,0.026327
20,0.004492,0.025783
21,0.004472,0.024970
22,0.004510,0.026167
23,0.004591,0.023671
24,0.003969,0.025839
25,0.003961,0.026817
26,0.004037,0.024682
27,0.003610,0.025854
28,0.003656,0.026025
29,0.003580,0.026356
30,0.003770,0.026824
31,0.003500,0.025530
32,0.003741,0.026009
33,0.003675,0.026208
34,0.003692,0.027457
35,0.003468,0.026065
36,0.003335,0.026126
37,0.003527,0.027208
38,0.003310,0.028075
39,0.003477,0.026553
40,0.003150,0.028597
41,0.003163,0.027464
42,0.003482,0.028284
43,0.003165,0.028215
44,0.003201,0.028690
45,0.003167,0.028687
46,0.003153,0.027571
47,0.003077,0.027098
48,0.003095,0.028342
49,0.003097,0.027073


==> data_recalls_forest_except_with_local_csv.tex <==
regions,i,recall,bw,rtt,loss,jitter,net,load,all,bw_err,rtt_err,loss_err,jitter_err,net_err,load_err,all_err
1,0,1,1.000,1.000,0.968,0.970,1.000,0.997,0.992,0.000,0.001,0.009,0.015,0.000,0.003,0.002
1,1,3,1.000,1.000,1.000,0.999,1.000,0.998,0.999,0.000,0.000,0.000,0.001,0.000,0.002,0.001
1,2,5,1.000,1.000,1.000,1.000,1.000,0.998,0.999,0.000,0.000,0.000,0.000,0.000,0.002,0.001
1,3,10,1.000,1.000,1.000,1.000,1.000,0.998,0.999,0.000,0.000,0.000,0.000,0.000,0.002,0.001
2,0,1,1.000,0.999,0.963,0.976,1.000,0.998,0.993,0.000,0.001,0.005,0.005,0.000,0.001,0.001
2,1,3,1.000,1.000,1.000,1.000,1.000,0.999,1.000,0.000,0.000,0.000,0.000,0.000,0.001,0.000
2,2,5,1.000,1.000,1.000,1.000,1.000,0.999,1.000,0.000,0.000,0.000,0.000,0.000,0.001,0.000
2,3,10,1.000,1.000,1.000,1.000,1.000,0.999,1.000,0.000,0.000,0.000,0.000,0.000,0.001,0.000
3,0,1,1.000,0.998,0.959,0.977,1.000,0.999,0.992,0.000,0.000,0.004,0.003,0.000,0.000,0.000
3,1,3,1.000,1.000,1.000,1.000,1.000,1.000,1.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
3,2,5,1.000,1.000,1.000,1.000,1.000,1.000,1.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
3,3,10,1.000,1.000,1.000,1.000,1.000,1.000,1.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
4,0,1,1.000,0.997,0.953,0.976,1.000,0.999,0.992,0.000,0.000,0.002,0.002,0.000,0.000,0.000
4,1,3,1.000,1.000,1.000,1.000,1.000,1.000,1.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
4,2,5,1.000,1.000,1.000,1.000,1.000,1.000,1.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
4,3,10,1.000,1.000,1.000,1.000,1.000,1.000,1.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
5,0,1,1.000,0.997,0.949,0.975,1.000,0.999,0.991,0.000,0.000,0.002,0.001,0.000,0.000,0.000
5,1,3,1.000,1.000,1.000,1.000,1.000,1.000,1.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
5,2,5,1.000,1.000,1.000,1.000,1.000,1.000,1.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
5,3,10,1.000,1.000,1.000,1.000,1.000,1.000,1.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
6,0,1,1.000,0.997,0.945,0.974,1.000,1.000,0.991,0.000,0.000,0.002,0.001,0.000,0.000,0.000
6,1,3,1.000,1.000,1.000,1.000,1.000,1.000,1.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
6,2,5,1.000,1.000,1.000,1.000,1.000,1.000,1.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
6,3,10,1.000,1.000,1.000,1.000,1.000,1.000,1.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
7,0,1,1.000,0.997,0.942,0.972,1.000,1.000,0.990,0.000,0.000,0.002,0.001,0.000,0.000,0.000
7,1,3,1.000,1.000,1.000,1.000,1.000,1.000,1.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
7,2,5,1.000,1.000,1.000,1.000,1.000,1.000,1.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
7,3,10,1.000,1.000,1.000,1.000,1.000,1.000,1.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
8,0,1,1.000,0.997,0.940,0.973,1.000,1.000,0.990,0.000,0.000,0.003,0.001,0.000,0.000,0.000
8,1,3,1.000,1.000,1.000,1.000,1.000,1.000,1.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
8,2,5,1.000,1.000,1.000,1.000,1.000,1.000,1.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
8,3,10,1.000,1.000,1.000,1.000,1.000,1.000,1.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
9,0,1,1.000,0.996,0.937,0.972,1.000,1.000,0.989,0.000,0.001,0.004,0.002,0.000,0.000,0.001
9,1,3,1.000,1.000,1.000,1.000,1.000,1.000,1.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
9,2,5,1.000,1.000,1.000,1.000,1.000,1.000,1.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
9,3,10,1.000,1.000,1.000,1.000,1.000,1.000,1.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
10,0,1,1.000,0.996,0.935,0.966,1.000,1.000,0.989,0.000,0.001,0.007,0.004,0.000,0.000,0.001
10,1,3,1.000,1.000,1.000,0.999,1.000,1.000,1.000,0.000,0.000,0.000,0.001,0.000,0.000,0.000
10,2,5,1.000,1.000,1.000,1.000,1.000,1.000,1.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
10,3,10,1.000,1.000,1.000,1.000,1.000,1.000,1.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000


==> data_recalls_forest_only_csv.tex <==
regions,i,recall,bw,rtt,loss,jitter,net,load,all,bw_err,rtt_err,loss_err,jitter_err,net_err,load_err,all_err
1,0,1,0.000,0.000,0.000,0.000,nan,nan,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
1,1,3,0.001,0.000,0.000,0.000,nan,nan,0.000,0.002,0.000,0.000,0.000,0.000,0.000,0.000
1,2,5,0.001,0.000,0.000,0.000,nan,nan,0.000,0.002,0.000,0.000,0.000,0.000,0.000,0.000
1,3,10,0.001,0.004,0.510,0.484,nan,nan,0.119,0.002,0.003,0.073,0.065,0.000,0.000,0.015
2,0,1,0.000,0.000,0.000,0.000,nan,nan,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
2,1,3,0.005,0.000,0.000,0.000,nan,nan,0.000,0.007,0.000,0.000,0.000,0.000,0.000,0.001
2,2,5,0.005,0.000,0.000,0.000,nan,nan,0.000,0.007,0.000,0.000,0.000,0.000,0.000,0.001
2,3,10,0.005,0.011,0.511,0.490,nan,nan,0.123,0.007,0.003,0.024,0.016,0.000,0.000,0.005
3,0,1,0.000,0.000,0.000,0.000,nan,nan,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
3,1,3,0.007,0.000,0.000,0.000,nan,nan,0.001,0.005,0.000,0.000,0.000,0.000,0.000,0.001
3,2,5,0.007,0.000,0.000,0.000,nan,nan,0.001,0.005,0.000,0.000,0.000,0.000,0.000,0.001
3,3,10,0.007,0.015,0.507,0.490,nan,nan,0.125,0.005,0.002,0.014,0.008,0.000,0.000,0.003
4,0,1,0.000,0.000,0.000,0.000,nan,nan,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
4,1,3,0.014,0.000,0.000,0.000,nan,nan,0.002,0.004,0.000,0.000,0.000,0.000,0.000,0.000
4,2,5,0.014,0.000,0.000,0.000,nan,nan,0.002,0.004,0.000,0.000,0.000,0.000,0.000,0.000
4,3,10,0.014,0.016,0.499,0.490,nan,nan,0.125,0.004,0.002,0.009,0.005,0.000,0.000,0.002
5,0,1,0.000,0.000,0.000,0.000,nan,nan,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
5,1,3,0.037,0.000,0.000,0.000,nan,nan,0.004,0.006,0.000,0.000,0.000,0.000,0.000,0.001
5,2,5,0.037,0.000,0.000,0.000,nan,nan,0.004,0.006,0.000,0.000,0.000,0.000,0.000,0.001
5,3,10,0.037,0.014,0.479,0.490,nan,nan,0.125,0.006,0.001,0.008,0.003,0.000,0.000,0.001
6,0,1,0.000,0.000,0.000,0.000,nan,nan,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
6,1,3,0.052,0.000,0.000,0.000,nan,nan,0.006,0.008,0.000,0.000,0.000,0.000,0.000,0.001
6,2,5,0.052,0.000,0.000,0.000,nan,nan,0.006,0.008,0.000,0.000,0.000,0.000,0.000,0.001
6,3,10,0.052,0.011,0.465,0.490,nan,nan,0.122,0.008,0.001,0.009,0.003,0.000,0.000,0.001
7,0,1,0.000,0.000,0.000,0.000,nan,nan,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
7,1,3,0.078,0.000,0.000,0.000,nan,nan,0.009,0.012,0.000,0.000,0.000,0.000,0.000,0.001
7,2,5,0.078,0.000,0.000,0.000,nan,nan,0.009,0.012,0.000,0.000,0.000,0.000,0.000,0.001
7,3,10,0.078,0.009,0.439,0.490,nan,nan,0.121,0.012,0.001,0.013,0.003,0.000,0.000,0.001
8,0,1,0.000,0.000,0.000,0.000,nan,nan,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
8,1,3,0.111,0.000,0.000,0.000,nan,nan,0.012,0.023,0.000,0.000,0.000,0.000,0.000,0.003
8,2,5,0.111,0.000,0.000,0.000,nan,nan,0.012,0.023,0.000,0.000,0.000,0.000,0.000,0.003
8,3,10,0.111,0.006,0.405,0.490,nan,nan,0.119,0.023,0.001,0.024,0.004,0.000,0.000,0.002
9,0,1,0.000,0.000,0.000,0.000,nan,nan,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
9,1,3,0.168,0.000,0.000,0.000,nan,nan,0.018,0.034,0.000,0.000,0.000,0.000,0.000,0.004
9,2,5,0.168,0.000,0.000,0.000,nan,nan,0.018,0.034,0.000,0.000,0.000,0.000,0.000,0.004
9,3,10,0.168,0.004,0.353,0.490,nan,nan,0.118,0.034,0.001,0.033,0.003,0.000,0.000,0.002
10,0,1,0.000,0.000,0.000,0.000,nan,nan,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
10,1,3,0.180,0.000,0.000,0.000,nan,nan,0.020,0.100,0.000,0.000,0.000,0.000,0.000,0.011
10,2,5,0.180,0.000,0.000,0.000,nan,nan,0.020,0.100,0.000,0.000,0.000,0.000,0.000,0.011
10,3,10,0.180,0.003,0.325,0.490,nan,nan,0.115,0.100,0.001,0.101,0.000,0.000,0.000,0.003


==> data_recalls_gaussian_except_with_local_csv.tex <==
regions,i,recall,bw,rtt,loss,jitter,net,load,all,bw_err,rtt_err,loss_err,jitter_err,net_err,load_err,all_err
1,0,1,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
1,1,3,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
1,2,5,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
1,3,10,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
2,0,1,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
2,1,3,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
2,2,5,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
2,3,10,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
3,0,1,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
3,1,3,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
3,2,5,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
3,3,10,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
4,0,1,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
4,1,3,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
4,2,5,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
4,3,10,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
5,0,1,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
5,1,3,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
5,2,5,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
5,3,10,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
6,0,1,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
6,1,3,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
6,2,5,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
6,3,10,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
7,0,1,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
7,1,3,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
7,2,5,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
7,3,10,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
8,0,1,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
8,1,3,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
8,2,5,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
8,3,10,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
9,0,1,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
9,1,3,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
9,2,5,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
9,3,10,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
10,0,1,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
10,1,3,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
10,2,5,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000
10,3,10,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000,0.000


==> data_recalls_gaussian_only_csv.tex <==
regions,i,recall,bw,rtt,loss,jitter,net,load,all,bw_err,rtt_err,loss_err,jitter_err,net_err,load_err,all_err
1,0,1,0.000,0.000,0.000,0.023,nan,nan,0.002,0.000,0.000,0.000,0.043,0.000,0.000,0.004
1,1,3,0.000,0.013,0.004,0.109,nan,nan,0.020,0.000,0.029,0.010,0.164,0.000,0.000,0.023
1,2,5,0.000,0.023,0.018,0.227,nan,nan,0.040,0.000,0.045,0.021,0.192,0.000,0.000,0.029
1,3,10,0.000,0.717,0.306,0.950,nan,nan,0.616,0.000,0.222,0.209,0.087,0.000,0.000,0.158
2,0,1,0.000,0.000,0.010,0.142,nan,nan,0.018,0.000,0.001,0.009,0.043,0.000,0.000,0.005
2,1,3,0.000,0.045,0.089,0.247,nan,nan,0.069,0.000,0.015,0.040,0.060,0.000,0.000,0.019
2,2,5,0.000,0.166,0.107,0.332,nan,nan,0.160,0.000,0.045,0.045,0.060,0.000,0.000,0.038
2,3,10,0.000,0.673,0.390,0.899,nan,nan,0.593,0.000,0.047,0.068,0.037,0.000,0.000,0.035
3,0,1,0.000,0.000,0.016,0.184,nan,nan,0.023,0.000,0.000,0.005,0.021,0.000,0.000,0.003
3,1,3,0.000,0.052,0.147,0.318,nan,nan,0.088,0.000,0.006,0.025,0.035,0.000,0.000,0.010
3,2,5,0.000,0.225,0.174,0.402,nan,nan,0.215,0.000,0.025,0.029,0.033,0.000,0.000,0.022
3,3,10,0.000,0.673,0.410,0.848,nan,nan,0.589,0.000,0.023,0.033,0.021,0.000,0.000,0.019
4,0,1,0.000,0.000,0.018,0.207,nan,nan,0.026,0.000,0.000,0.003,0.013,0.000,0.000,0.002
4,1,3,0.000,0.057,0.180,0.350,nan,nan,0.099,0.000,0.004,0.018,0.024,0.000,0.000,0.006
4,2,5,0.000,0.249,0.211,0.435,nan,nan,0.238,0.000,0.017,0.021,0.023,0.000,0.000,0.015
4,3,10,0.000,0.671,0.405,0.810,nan,nan,0.582,0.000,0.015,0.020,0.016,0.000,0.000,0.013
5,0,1,0.000,0.000,0.019,0.218,nan,nan,0.027,0.000,0.000,0.002,0.010,0.000,0.000,0.001
5,1,3,0.000,0.059,0.193,0.356,nan,nan,0.102,0.000,0.003,0.015,0.020,0.000,0.000,0.005
5,2,5,0.000,0.249,0.223,0.442,nan,nan,0.240,0.000,0.014,0.018,0.018,0.000,0.000,0.013
5,3,10,0.000,0.662,0.392,0.776,nan,nan,0.571,0.000,0.011,0.016,0.014,0.000,0.000,0.010
6,0,1,0.000,0.000,0.019,0.222,nan,nan,0.028,0.000,0.000,0.002,0.009,0.000,0.000,0.001
6,1,3,0.000,0.060,0.191,0.345,nan,nan,0.101,0.000,0.003,0.014,0.020,0.000,0.000,0.005
6,2,5,0.000,0.234,0.217,0.436,nan,nan,0.229,0.000,0.014,0.018,0.017,0.000,0.000,0.013
6,3,10,0.000,0.651,0.372,0.747,nan,nan,0.558,0.000,0.011,0.015,0.013,0.000,0.000,0.010
7,0,1,0.000,0.000,0.019,0.223,nan,nan,0.028,0.000,0.000,0.002,0.009,0.000,0.000,0.001
7,1,3,0.000,0.060,0.179,0.326,nan,nan,0.098,0.000,0.003,0.017,0.023,0.000,0.000,0.005
7,2,5,0.000,0.212,0.200,0.421,nan,nan,0.211,0.000,0.017,0.022,0.020,0.000,0.000,0.016
7,3,10,0.000,0.640,0.345,0.724,nan,nan,0.545,0.000,0.012,0.017,0.015,0.000,0.000,0.011
8,0,1,0.000,0.000,0.019,0.223,nan,nan,0.028,0.000,0.000,0.003,0.012,0.000,0.000,0.001
8,1,3,0.000,0.062,0.165,0.304,nan,nan,0.094,0.000,0.004,0.023,0.031,0.000,0.000,0.007
8,2,5,0.000,0.189,0.178,0.403,nan,nan,0.191,0.000,0.024,0.030,0.027,0.000,0.000,0.022
8,3,10,0.000,0.631,0.319,0.702,nan,nan,0.534,0.000,0.016,0.024,0.020,0.000,0.000,0.014
9,0,1,0.000,0.000,0.019,0.224,nan,nan,0.028,0.000,0.000,0.005,0.019,0.000,0.000,0.002
9,1,3,0.000,0.064,0.149,0.282,nan,nan,0.092,0.000,0.008,0.040,0.054,0.000,0.000,0.012
9,2,5,0.000,0.169,0.156,0.392,nan,nan,0.174,0.000,0.043,0.054,0.046,0.000,0.000,0.040
9,3,10,0.000,0.626,0.294,0.683,nan,nan,0.526,0.000,0.026,0.043,0.036,0.000,0.000,0.024
10,0,1,0.000,0.000,0.020,0.225,nan,nan,0.028,0.000,0.000,0.000,0.000,0.000,0.000,0.000
10,1,3,0.000,0.068,0.133,0.258,nan,nan,0.090,0.000,0.000,0.000,0.000,0.000,0.000,0.000
10,2,5,0.000,0.154,0.133,0.384,nan,nan,0.161,0.000,0.000,0.000,0.000,0.000,0.000,0.000
10,3,10,0.000,0.614,0.267,0.662,nan,nan,0.512,0.000,0.000,0.000,0.000,0.000,0.000,0.000


==> data_recalls_hybrid3p_except_with_local_csv.tex <==
regions,i,recall,bw,rtt,loss,jitter,net,load,all,bw_err,rtt_err,loss_err,jitter_err,net_err,load_err,all_err
1,0,1,0.982,0.987,0.860,0.830,0.988,0.984,0.958,0.016,0.007,0.028,0.045,0.015,0.010,0.008
1,1,3,0.997,0.999,0.986,0.978,0.998,0.996,0.995,0.005,0.001,0.005,0.011,0.003,0.004,0.002
1,2,5,0.998,1.000,0.995,0.995,0.998,0.999,0.998,0.005,0.000,0.003,0.004,0.003,0.002,0.001
1,3,10,1.000,1.000,0.999,0.997,0.998,0.999,0.999,0.000,0.000,0.002,0.003,0.002,0.001,0.001
2,0,1,0.984,0.954,0.843,0.871,0.971,0.990,0.948,0.004,0.009,0.012,0.013,0.009,0.002,0.005
2,1,3,0.998,0.992,0.975,0.978,0.997,0.994,0.991,0.001,0.003,0.004,0.004,0.002,0.002,0.002
2,2,5,0.999,0.997,0.992,0.993,0.997,0.996,0.996,0.001,0.001,0.002,0.002,0.001,0.001,0.001
2,3,10,1.000,0.999,0.998,0.998,0.997,0.998,0.998,0.000,0.000,0.001,0.001,0.001,0.001,0.000
3,0,1,0.983,0.930,0.816,0.852,0.972,0.991,0.938,0.004,0.011,0.015,0.016,0.014,0.002,0.005
3,1,3,0.997,0.984,0.969,0.974,0.998,0.995,0.988,0.001,0.004,0.006,0.004,0.001,0.002,0.002
3,2,5,0.999,0.995,0.991,0.992,0.998,0.997,0.995,0.001,0.002,0.003,0.002,0.001,0.001,0.001
3,3,10,0.999,0.998,0.998,0.997,0.998,0.999,0.998,0.001,0.001,0.001,0.001,0.001,0.001,0.000
4,0,1,0.986,0.901,0.799,0.831,0.973,0.991,0.927,0.003,0.010,0.011,0.011,0.009,0.002,0.004
4,1,3,0.999,0.979,0.965,0.963,0.997,0.995,0.984,0.000,0.004,0.004,0.005,0.001,0.001,0.002
4,2,5,0.999,0.994,0.989,0.988,0.997,0.996,0.994,0.000,0.001,0.002,0.002,0.001,0.001,0.001
4,3,10,1.000,0.998,0.998,0.994,0.997,0.999,0.998,0.000,0.001,0.001,0.001,0.001,0.000,0.000
5,0,1,0.982,0.874,0.785,0.805,0.963,0.990,0.914,0.002,0.009,0.009,0.011,0.008,0.001,0.004
5,1,3,0.998,0.970,0.960,0.952,0.995,0.994,0.980,0.001,0.004,0.004,0.005,0.002,0.001,0.002
5,2,5,0.999,0.991,0.987,0.983,0.995,0.995,0.992,0.000,0.001,0.002,0.002,0.001,0.001,0.001
5,3,10,0.999,0.997,0.997,0.993,0.995,0.998,0.997,0.000,0.000,0.001,0.001,0.001,0.000,0.000
6,0,1,0.984,0.860,0.773,0.803,0.968,0.991,0.910,0.002,0.009,0.009,0.009,0.007,0.001,0.004
6,1,3,0.997,0.964,0.957,0.950,0.996,0.994,0.978,0.001,0.004,0.004,0.004,0.001,0.001,0.002
6,2,5,0.999,0.990,0.987,0.982,0.997,0.996,0.992,0.000,0.001,0.002,0.002,0.001,0.001,0.001
6,3,10,0.999,0.997,0.997,0.992,0.997,0.999,0.997,0.000,0.001,0.001,0.001,0.001,0.000,0.000
7,0,1,0.984,0.836,0.752,0.787,0.958,0.991,0.898,0.003,0.011,0.013,0.012,0.011,0.001,0.005
7,1,3,0.998,0.956,0.949,0.942,0.996,0.994,0.974,0.001,0.005,0.005,0.006,0.002,0.001,0.002
7,2,5,0.999,0.988,0.984,0.979,0.996,0.996,0.991,0.000,0.002,0.003,0.003,0.001,0.001,0.001
7,3,10,1.000,0.997,0.997,0.991,0.997,0.999,0.997,0.000,0.001,0.001,0.002,0.001,0.000,0.000
8,0,1,0.984,0.813,0.738,0.778,0.951,0.990,0.888,0.002,0.007,0.007,0.007,0.007,0.001,0.003
8,1,3,0.996,0.948,0.950,0.934,0.996,0.994,0.971,0.001,0.003,0.003,0.003,0.001,0.001,0.001
8,2,5,0.999,0.986,0.985,0.977,0.996,0.996,0.990,0.000,0.001,0.001,0.002,0.001,0.000,0.001
8,3,10,0.999,0.997,0.996,0.992,0.997,0.999,0.997,0.000,0.000,0.001,0.001,0.001,0.000,0.000
9,0,1,0.985,0.790,0.709,0.768,0.950,0.990,0.878,0.003,0.013,0.016,0.013,0.013,0.001,0.005
9,1,3,0.996,0.936,0.946,0.931,0.996,0.994,0.967,0.001,0.007,0.006,0.007,0.001,0.001,0.003
9,2,5,0.998,0.982,0.982,0.976,0.997,0.996,0.989,0.001,0.002,0.003,0.004,0.001,0.001,0.001
9,3,10,0.999,0.995,0.996,0.992,0.997,0.998,0.997,0.000,0.001,0.001,0.002,0.001,0.001,0.001
10,0,1,0.982,0.789,0.701,0.762,0.961,0.992,0.878,0.005,0.030,0.020,0.036,0.024,0.003,0.011
10,1,3,0.997,0.942,0.946,0.934,0.998,0.995,0.970,0.003,0.015,0.014,0.016,0.003,0.002,0.006
10,2,5,0.998,0.982,0.982,0.978,0.998,0.997,0.990,0.003,0.008,0.004,0.007,0.003,0.002,0.003
10,3,10,0.999,0.996,0.996,0.994,0.998,0.999,0.997,0.002,0.002,0.002,0.004,0.003,0.001,0.001


==> data_recalls_hybrid3p_only_csv.tex <==
regions,i,recall,bw,rtt,loss,jitter,net,load,all,bw_err,rtt_err,loss_err,jitter_err,net_err,load_err,all_err
1,0,1,0.096,0.333,0.060,0.084,nan,nan,0.255,0.045,0.041,0.023,0.032,0.000,0.000,0.031
1,1,3,0.152,0.491,0.185,0.202,nan,nan,0.391,0.061,0.046,0.047,0.048,0.000,0.000,0.036
1,2,5,0.192,0.530,0.216,0.240,nan,nan,0.429,0.065,0.046,0.051,0.054,0.000,0.000,0.036
1,3,10,0.265,0.575,0.451,0.478,nan,nan,0.521,0.074,0.047,0.050,0.080,0.000,0.000,0.034
2,0,1,0.170,0.281,0.026,0.048,nan,nan,0.212,0.023,0.017,0.005,0.009,0.000,0.000,0.012
2,1,3,0.243,0.442,0.087,0.118,nan,nan,0.342,0.026,0.019,0.012,0.015,0.000,0.000,0.014
2,2,5,0.291,0.494,0.113,0.150,nan,nan,0.388,0.029,0.020,0.014,0.016,0.000,0.000,0.015
2,3,10,0.395,0.584,0.389,0.405,nan,nan,0.520,0.034,0.020,0.018,0.021,0.000,0.000,0.015
3,0,1,0.124,0.319,0.035,0.038,nan,nan,0.232,0.023,0.020,0.009,0.009,0.000,0.000,0.013
3,1,3,0.199,0.500,0.103,0.092,nan,nan,0.375,0.029,0.020,0.016,0.016,0.000,0.000,0.015
3,2,5,0.258,0.568,0.132,0.123,nan,nan,0.433,0.034,0.021,0.018,0.019,0.000,0.000,0.016
3,3,10,0.374,0.676,0.395,0.357,nan,nan,0.574,0.040,0.020,0.023,0.025,0.000,0.000,0.016
4,0,1,0.150,0.311,0.034,0.033,nan,nan,0.230,0.018,0.013,0.006,0.006,0.000,0.000,0.009
4,1,3,0.242,0.510,0.115,0.080,nan,nan,0.386,0.021,0.013,0.011,0.009,0.000,0.000,0.009
4,2,5,0.305,0.585,0.153,0.107,nan,nan,0.450,0.024,0.013,0.013,0.011,0.000,0.000,0.010
4,3,10,0.422,0.702,0.411,0.328,nan,nan,0.594,0.029,0.013,0.017,0.017,0.000,0.000,0.010
5,0,1,0.145,0.298,0.037,0.030,nan,nan,0.220,0.014,0.012,0.006,0.005,0.000,0.000,0.008
5,1,3,0.252,0.499,0.125,0.068,nan,nan,0.379,0.018,0.012,0.011,0.008,0.000,0.000,0.008
5,2,5,0.310,0.577,0.168,0.097,nan,nan,0.446,0.020,0.011,0.012,0.010,0.000,0.000,0.008
5,3,10,0.421,0.705,0.432,0.310,nan,nan,0.597,0.023,0.011,0.015,0.014,0.000,0.000,0.008
6,0,1,0.159,0.290,0.040,0.021,nan,nan,0.216,0.015,0.011,0.005,0.003,0.000,0.000,0.008
6,1,3,0.282,0.494,0.134,0.053,nan,nan,0.379,0.021,0.011,0.011,0.006,0.000,0.000,0.008
6,2,5,0.338,0.576,0.173,0.075,nan,nan,0.447,0.023,0.010,0.013,0.007,0.000,0.000,0.008
6,3,10,0.443,0.708,0.437,0.295,nan,nan,0.600,0.025,0.009,0.015,0.012,0.000,0.000,0.008
7,0,1,0.171,0.279,0.035,0.021,nan,nan,0.210,0.020,0.014,0.006,0.004,0.000,0.000,0.010
7,1,3,0.321,0.483,0.123,0.056,nan,nan,0.375,0.026,0.013,0.013,0.008,0.000,0.000,0.010
7,2,5,0.376,0.563,0.165,0.081,nan,nan,0.442,0.028,0.012,0.014,0.009,0.000,0.000,0.010
7,3,10,0.471,0.696,0.419,0.300,nan,nan,0.594,0.030,0.012,0.020,0.016,0.000,0.000,0.010
8,0,1,0.244,0.273,0.036,0.021,nan,nan,0.214,0.019,0.009,0.005,0.003,0.000,0.000,0.006
8,1,3,0.403,0.482,0.124,0.055,nan,nan,0.384,0.022,0.008,0.009,0.006,0.000,0.000,0.006
8,2,5,0.463,0.562,0.166,0.078,nan,nan,0.450,0.022,0.008,0.011,0.007,0.000,0.000,0.006
8,3,10,0.560,0.686,0.416,0.295,nan,nan,0.597,0.022,0.007,0.015,0.011,0.000,0.000,0.006
9,0,1,0.283,0.280,0.025,0.020,nan,nan,0.222,0.031,0.018,0.006,0.007,0.000,0.000,0.012
9,1,3,0.462,0.478,0.114,0.052,nan,nan,0.386,0.030,0.017,0.016,0.011,0.000,0.000,0.012
9,2,5,0.516,0.554,0.157,0.074,nan,nan,0.449,0.032,0.016,0.018,0.014,0.000,0.000,0.012
9,3,10,0.615,0.676,0.398,0.294,nan,nan,0.594,0.037,0.014,0.025,0.021,0.000,0.000,0.011
10,0,1,0.351,0.283,0.014,0.017,nan,nan,0.229,0.054,0.037,0.009,0.012,0.000,0.000,0.024
10,1,3,0.557,0.477,0.091,0.049,nan,nan,0.393,0.059,0.028,0.028,0.021,0.000,0.000,0.022
10,2,5,0.590,0.562,0.139,0.070,nan,nan,0.460,0.066,0.030,0.042,0.030,0.000,0.000,0.025
10,3,10,0.684,0.690,0.343,0.287,nan,nan,0.604,0.059,0.029,0.073,0.048,0.000,0.000,0.024


==> data_region_recall_csv.tex <==
i,family,forest,forest_err,gaussian,gaussian_err,diagnet,diagnet_err,hybrid3,hybrid3_err,hybrid3p,hybrid3p_err
1,ovh-gravelines,0.038,0.021,0.021,0.000,0.403,0.029,0.401,0.025,0.410,0.028
2,vultr-seattle,0.000,0.000,0.164,0.000,0.359,0.032,0.360,0.026,0.374,0.023
3,ovh-singapore,0.999,0.001,0.000,0.000,0.621,0.046,0.677,0.065,0.946,0.022
4,ovh-beauharnois,1.000,0.000,0.000,0.000,0.486,0.022,0.611,0.023,0.949,0.012
5,scw-amsterdam,1.000,0.000,0.000,0.000,0.460,0.051,0.652,0.040,0.967,0.012
6,net-edge,1.000,0.000,0.000,0.000,0.865,0.064,0.851,0.061,0.998,0.003

